Safe Handover in Mixed-Initiative Control for Cyber-Physical Systems

For mixed-initiative control between cyber-physical systems (CPS) and its users, it is still an open question how machines can safely hand over control to humans. In this work, we propose a concept to provide technological support that uses formal methods from AI -- description logic (DL) and automated planning -- to predict more reliably when a hand-over is necessary, and to increase the advance notice for handovers by planning ahead of runtime. We combine this with methods from human-computer interaction (HCI) and natural language generation (NLG) to develop solutions for safe and smooth handovers and provide an example autonomous driving scenario. A study design is proposed with the assessment of qualitative feedback, cognitive load and trust in automation.

==> metrics_study.tex <==
\newcommand{\cwptaktilavg}{1989.61}
\newcommand{\cwpnoanswershard}{10}
\newcommand{\cwpaudiostdhard}{545.16}
\newcommand{\cwpnoanswerseasy}{4}
\newcommand{\cwptaktilavgeasy}{1804.0}
\newcommand{\cwpvisuellavghard}{2718.93}
\newcommand{\cwpstddevage}{11.74}
\newcommand{\cwpaudioavg}{2230.53}
\newcommand{\cwptotalcues}{216}
\newcommand{\cwpvisuellstdeasy}{1236.01}
\newcommand{\cwpaudiostd}{600.37}
\newcommand{\cwpvisuellstdhard}{1332.19}
\newcommand{\cwpcueshard }{{'taktil': {1: {'std': 490.93931368573675, 'avg': 1920.4166666666667}, 2: {'std': 444.47738835663012, 'avg': 2277.181818181818}, 3: {'std': 643.13740289946168, 'avg': 2368.090909090909}}, 'visuell': {1: {'std': 1334.5854768660299, 'avg': 3004.7777777777778}, 2: {'std': 890.86822726321725, 'avg': 2550.7272727272725}, 3: {'std': 1725.5726540412606, 'avg': 2628.625}}, 'audio': {1: {'std': 593.19677150353937, 'avg': 2253.5833333333335}, 2: {'std': 593.61750568489424, 'avg': 2254.9166666666665}, 3: {'std': 432.82450895894931, 'avg': 2252.6666666666665}}}}
\newcommand{\cwpcueseasy }{{'taktil': {1: {'std': 592.42736896601934, 'avg': 1754.25}, 2: {'std': 640.55124761914738, 'avg': 1642.090909090909}, 3: {'std': 1.771690968789108, 'avg': 2002.1666666666667}}, 'visuell': {1: {'std': 1000.3047985489223, 'avg': 2004.9000000000001}, 2: {'std': 1419.0628032858242, 'avg': 2276.181818181818}, 3: {'std': 1196.2606037560399, 'avg': 1892.1111111111111}}, 'audio': {1: {'std': 696.45173397119163, 'avg': 2234.4615384615386}, 2: {'std': 694.75401972856127, 'avg': 2234.9230769230771}, 3: {'std': 531.02064279736157, 'avg': 2158.0}}}}
\newcommand{\cwpvisuellstd}{1323.61}
\newcommand{\cwpmaxage}{60}
\newcommand{\cwpaudiostdeasy}{646.43}
\newcommand{\cwptaktilstdhard}{566.64}
\newcommand{\cwptotalwronganswers}{4}
\newcommand{\cwpwronganwershard}{4}
\newcommand{\cwpvisuellavgeasy}{2070.53}
\newcommand{\cwpaudioavgeasy}{2209.13}
\newcommand{\cwpclimbinghigh}{5}
\newcommand{\cwpclimbingmedium}{7}
\newcommand{\cwptotalcorrectanswers}{198}
\newcommand{\cwptaktilstdeasy}{521.38}
\newcommand{\cwpvisuellavg}{2383.55}
\newcommand{\cwptaktilstd}{575.82}
\newcommand{\cwpscoretaktil }{29}
\newcommand{\cwpscorevisuell }{11}
\newcommand{\cwpscoreequal }{6}
\newcommand{\cwpscoreaudio }{26}
\newcommand{\cwpnumberparticipants}{12}
\newcommand{\cwpnumberfemale}{1}
\newcommand{\cwpaudioavghard}{2253.72}
\newcommand{\cwpwronganwerseasy}{0}
\newcommand{\cwpminage}{13}
\newcommand{\cwptaktilavghard}{2180.68}
\newcommand{\cwpnumbermale}{11}
\newcommand{\cwptotalnoanswers}{14}
\newcommand{\cwpavgage}{34.58}
\newcommand{\cwpclimbinglow}{0}

